Design of Threshold-Constrained Indirect Quantizers

We address the problem of indirect quantization of a source subject to a mean-squared error distortion constraint. A well-known result of Wolf and Ziv is that the problem can be reduced to a standard (direct) quantization problem via a two-step approach: first apply the conditional expectation estimator, obtaining a ``new'' source, then solve for the optimal quantizer for the latter source. When quantization is implemented in hardware, however, invariably constraints on the allowable class of quantizers are imposed, typically limiting the class to \emph{time-invariant} scalar quantizers with contiguous quantization cells. In the present work, optimal indirect quantization subject to these constraints is considered. Necessary conditions an optimal quantizer within this class must satisfy are derived, in the form of generalized Lloyd-Max conditions, and an iterative algorithm for the design of such quantizers is proposed. Furthermore, for the case of a scalar observation, we derive a non-iterative algorithm for finding the optimal indirect quantizer based on dynamic programming.

==> Figs/Lloyd_Max_2D.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=2*0.75pt,y=2*0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,416); %set diagram left start at 0, and has height of 416

%Shape: Grid [id:dp34219463201848077] 
\draw  [draw opacity=0] (249.6,150.13) -- (350.13,150.13) -- (350.13,251.13) -- (249.6,251.13) -- cycle ; \draw   (249.6,150.13) -- (249.6,251.13)(269.6,150.13) -- (269.6,251.13)(289.6,150.13) -- (289.6,251.13)(309.6,150.13) -- (309.6,251.13)(329.6,150.13) -- (329.6,251.13)(349.6,150.13) -- (349.6,251.13) ; \draw   (249.6,150.13) -- (350.13,150.13)(249.6,170.13) -- (350.13,170.13)(249.6,190.13) -- (350.13,190.13)(249.6,210.13) -- (350.13,210.13)(249.6,230.13) -- (350.13,230.13)(249.6,250.13) -- (350.13,250.13) ; \draw    ;
%Straight Lines [id:da3035643011026934] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ]   (309.35,129.67) -- (309.75,270.47) ;
%Straight Lines [id:da4852304967912451] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ]   (369.92,190.17) -- (230.1,190.47) ;

% Text Node
\draw (253.58,235.15) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-0.39] [align=left] {$\displaystyle \hat{s}_{1,1}$};
% Text Node
\draw (273.8,236.27) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$\hat{s}_{2,1}$};
% Text Node
\draw (293.6,236.47) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 144; green, 19; blue, 254 }  ,opacity=1 ]  {$\hat{s}_{3,1}$};
% Text Node
\draw (314,235.27) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 144; green, 19; blue, 254 }  ,opacity=1 ]  {$\hat{s}_{4,1}$};
% Text Node
\draw (333.6,235.67) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$\hat{s}_{5,1}$};
% Text Node
\draw (253.58,215.95) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-0.39] [align=left] {$\displaystyle \hat{s}_{1,2}$};
% Text Node
\draw (273.8,216.07) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$\hat{s}_{2,2}$};
% Text Node
\draw (293.2,215.67) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 144; green, 19; blue, 254 }  ,opacity=1 ]  {$\hat{s}_{3,2}$};
% Text Node
\draw (313,216.07) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 144; green, 19; blue, 254 }  ,opacity=1 ]  {$\hat{s}_{4,2}$};
% Text Node
\draw (333.6,215.67) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$\hat{s}_{5,2}$};
% Text Node
\draw (253.58,195.55) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 144; green, 19; blue, 254 }  ,opacity=1 ,rotate=-0.39] [align=left] {$\displaystyle \hat{s}_{1,3}$};
% Text Node
\draw (273.8,195.87) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 144; green, 19; blue, 254 }  ,opacity=1 ]  {$\hat{s}_{2,3}$};
% Text Node
\draw (294,195.67) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 144; green, 19; blue, 254 }  ,opacity=1 ]  {$\hat{s}_{3,3}$};
% Text Node
\draw (313.6,195.67) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 144; green, 19; blue, 254 }  ,opacity=1 ]  {$\hat{s}_{4,3}$};
% Text Node
\draw (284.98,252.75) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-0.39] [align=left] {$\displaystyle t_{2}$};
% Text Node
\draw (265.38,253.15) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-0.39] [align=left] {$\displaystyle t_{1}$};
% Text Node
\draw (306.18,253.55) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-0.39] [align=left] {$\displaystyle t_{3}$};
% Text Node
\draw (325.98,252.35) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-0.39] [align=left] {$\displaystyle t_{4}$};
% Text Node
\draw (245.38,253.15) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-0.39] [align=left] {$\displaystyle t_{0}$};
% Text Node
\draw (345.78,251.95) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-0.39] [align=left] {$\displaystyle t_{5}$};
% Text Node
\draw (238.58,226.35) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-0.39] [align=left] {$\displaystyle t_{1}$};
% Text Node
\draw (238.18,207.15) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-0.39] [align=left] {$\displaystyle t_{2}$};
% Text Node
\draw (239.18,186.95) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-0.39] [align=left] {$\displaystyle t_{3}$};
% Text Node
\draw (238.78,166.55) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-0.39] [align=left] {$\displaystyle t_{4}$};
% Text Node
\draw (238.38,147.35) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,rotate=-0.39] [align=left] {$\displaystyle t_{5}$};
% Text Node
\draw (332.8,195.67) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 144; green, 19; blue, 254 }  ,opacity=1 ]  {$\hat{s}_{5,3}$};
% Text Node
\draw (333.55,176.47) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 144; green, 19; blue, 254 }  ,opacity=1 ]  {$\hat{s}_{5,4}$};
% Text Node
\draw (334.1,156.47) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$\hat{s}_{5,5}$};
% Text Node
\draw (313.2,176.07) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 144; green, 19; blue, 254 }  ,opacity=1 ]  {$\hat{s}_{4,4}$};
% Text Node
\draw (313.8,155.67) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 144; green, 19; blue, 254 }  ,opacity=1 ]  {$\hat{s}_{4,5}$};
% Text Node
\draw (294.2,155.87) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 144; green, 19; blue, 254 }  ,opacity=1 ]  {$\hat{s}_{3,5}$};
% Text Node
\draw (294.45,176.07) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 124; green, 0; blue, 255 }  ,opacity=1 ]  {$\hat{s}_{3,4}$};
% Text Node
\draw (274,175.87) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 144; green, 19; blue, 254 }  ,opacity=1 ]  {$\hat{s}_{2,4}$};
% Text Node
\draw (273.2,155.67) node [anchor=north west][inner sep=0.75pt]  [font=\tiny]  {$\hat{s}_{2,5}$};
% Text Node
\draw (253.98,175.35) node [anchor=north west][inner sep=0.75pt]  [font=\tiny,color={rgb, 255:red, 144; green, 19; blue, 254 }  ,opacity=1 ,rotate=-0.39] [align=left] {$\displaystyle \hat{s}_{1,4}$};
% Text Node
\draw (253.58,155.55) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,rotate=-0.39] [align=left] {$\displaystyle \hat{s}_{1,5}$};


\end{tikzpicture}


==> defs.tex <==
% TeX Defs

% The IEEEI style package
%\usepackage{spconf}

\usepackage[tbtags]{amsmath} % defines many math commands and
% \usepackage{commath}
                 % subequations environment, etc
\usepackage{amssymb}  % get, among others, blackboard bold fonts
                      % defines extra symbols like \gtreqless, etc
\usepackage{verbatim} % get comment environment, + new verbatim
\usepackage{amsxtra}  % get, eg, \accentedsymbol
%\usepackage{spacing}
\usepackage{comment}

% Includes harpoons
\usepackage{mathabx}

\usepackage{enumerate}
%\usepackage{enumitem}

\usepackage{amsfonts}
\usepackage{color}

%%% For subfigures
\usepackage{subfig}
\usepackage{caption}
%\usepackage{subcaption}

% For \smiley
\usepackage{wasysym}


%% Squeeze and order citations
\usepackage{cite}


% % Number only equations which are referred to in text
% \usepackage{mathtools}
% \mathtoolsset{showonlyrefs=true}
% % \mathtoolsset{showonlyrefs=false}

% THEOREM ENVIRONMENTS

\usepackage{amsthm}

% \theoremstyle{theorem}
\newtheorem{thm}{Theorem}%[section]
\newtheorem{lem}{Lemma}%[section]
\newtheorem{claim}{Claim}%[section]
\newtheorem{assert}{Assertion}%[section]
\newtheorem{cor}{Corollary}%[section]
\newtheorem{prop}{Proposition}%[section]

\theoremstyle{definition}
\newtheorem{defn}{Definition}%[section]
\newtheorem*{defn*}{Definition}
\newtheorem{scheme}{Scheme}%[section]
\newtheorem*{scheme*}{Scheme}
\newtheorem{example}{Example}%[section]
\newtheorem{algo}{Algorithm}%[section]

\theoremstyle{remark}
\newtheorem{remark}{Remark}%[section]


\newcommand\hmmax{0}
\newcommand\bmmax{0}
\usepackage{fdsymbol}
\newcommand{\indep}{\upvDash}
\newcommand{\dep}{\nupvDash}

\usepackage{tikz}
\usetikzlibrary{shapes,arrows,decorations.markings,positioning,calc}

\tikzstyle{plant} = [draw, fill=red!5, rectangle, 
    minimum height=3em, minimum width=6em]
\tikzstyle{block} = [draw, fill=blue!5, rectangle, 
    minimum height=3em, minimum width=18mm]
\tikzstyle{sum} = [draw, fill=yellow!10, circle, node distance=1cm]
\tikzstyle{coord} = [coordinate]
\tikzstyle{gain} = [draw, fill=red!5, regular polygon, regular polygon sides=3, shape border rotate=-90]
\tikzstyle{pinstyle} = [pin edge={to-,thick,black}]

\tikzstyle{BitPipe} = [thick, decoration={markings,mark=at position
   1 with {\arrow[semithick]{open triangle 60}}},
   double distance=1.4pt, shorten >= 5.5pt,
   preaction = {decorate},
   postaction = {draw,line width=1.4pt, white,shorten >= 4.5pt}]

% Fits dotted rectangles around a group of blocks
\usetikzlibrary{fit,backgrounds}

%% For URLs (links) etc.
\usepackage{hyperref}
% \usepackage{url}

\usepackage{epsfig, graphicx, psfrag}

%%%%%%%\usepackage{appendix}
%%%%%%%

\usepackage[mathcal]{euscript}
% Mathcal lower-case lettters
% \newenvironment{frcseries}{\fontfamily{frc}\selectfont}{}
% \newcommand{\textfrc}[1]{{\frcseries#1}}
% % \newcommand{\mathfrc}[1]{\text{\textfrc{#1}}}
% \newcommand{\mathfrc}[1]{\mbox{\frcshape #1}}
% \providecommand{\Ber}{\mB\textfrc{er}}
\usepackage[cal=boondox]{mathalfa}
\providecommand{\Ber}{\mathcal{Ber}}
\providecommand{\Ber}{\mathcal{Bin}}

%Change maximal number of matrix columns (default = 10)
\setcounter{MaxMatrixCols}{12}

%------------------------%
% Flags for Bibliography %
%------------------------%
% \renewcommand{\davidsstar}{*}
\newcommand{\khina}{A.~Khina}
\newcommand{\invited}{}
% \newcommand{\isi}[1]{\textbf{ISI citations = #1}}
% \newcommand{\isiincl}[2]{\textbf{ISI cites (incl.\ \citeConf{#2}) = #1}}
% \newcommand{\google}{\textbf{Google Scholar cites =\ }}
% \newcommand{\googleincl}[2]{\textbf{GS cites (incl.\ \citeConf{#2}) = #1}}
% \newcommand{\googleinclabs}[3]{\textbf{GS cites (incl.\ \citeConf{#2}, \citeAbs{#3}) = #1}}
\newcommand{\PI}{}
\newcommand{\Student}{}
\newcommand{\CoRes}{}
\newcommand{\MyStudent}{}

% REFERENCE ENVIRONMENTS

\providecommand{\thmref}[1]{Theorem~\ref{#1}}
\providecommand{\assertref}[1]{Assert.~\ref{#1}}
\providecommand{\exref}[1]{Ex.~\ref{#1}}
% \providecommand{\footref}[1]{Foot.~\ref{#1}}
\providecommand{\defnref}[1]{Def.~\ref{#1}}
\providecommand{\secref}[1]{Sec.~\ref{#1}}
\providecommand{\lemref}[1]{Lemma~\ref{#1}}
\providecommand{\propref}[1]{Prop.~\ref{#1}}
\providecommand{\remref}[1]{Rem.~\ref{#1}}
\providecommand{\figref}[1]{Fig.~\ref{#1}}
\providecommand{\corref}[1]{Cor.~\ref{#1}}
\providecommand{\appref}[1]{App.~\ref{#1}}
\providecommand{\assref}[1]{Assump.~\ref{#1}}
\providecommand{\claimref}[1]{Claim~\ref{#1}}
\providecommand{\itmref}[1]{{\ref{#1}.}}
\providecommand{\algoref}[1]{Alg.~\ref{#1}}
\providecommand{\schemeref}[1]{Sch.~\ref{#1}}
\providecommand{\tabref}[1]{Tab.~\ref{#1}}
%\providecommand{\ccaption}{\caption*~{Figure~\thefigure: }}


\usepackage{refcount}
\providecommand{\footref}[1]{\footnotemark[\getrefnumber{#1}]}

\newcommand{\ie}{i.e.}
\newcommand{\iid}{i.i.d.}
\newcommand{\eg}{e.g.}
\newcommand{\etc}{etc.}
\newcommand{\viz}{viz.}
\newcommand{\etal}{\emph{et al.}}
\newcommand{\cf}{cf.}

\newcommand{\argsort}{\text{argsort}}

\newcommand{\reals}{\mathbb{R}}
\newcommand{\ints}{\mathbb{Z}}
\newcommand{\compls}{\mathbb{C}}
\newcommand{\nats}{\mathbb{N}}
\newcommand{\rats}{\mathbb{Q}}
\newcommand{\ltwor}{L^2(\reals)}
\newcommand{\ltwoz}{\ell^2(\ints)}
\newcommand{\ltwow}{L^2(\Omega)}

\newcommand{\ceil}[1]{\lceil{#1}\rceil}
\newcommand{\floor}[1]{\lfloor{#1}\rfloor}
\newcommand{\phase}{\measuredangle}


\DeclareMathOperator{\R}{Re}
\DeclareMathOperator{\I}{Im}
\DeclareMathOperator{\plog}{log^+}

\let\limsup\relax
\DeclareMathOperator*{\limsup}{\overline{lim}}
\let\liminf\relax
\DeclareMathOperator*{\liminf}{\underline{lim}}
\DeclareMathOperator*{\argmax}{arg\, max}
\DeclareMathOperator*{\argmin}{arg\, min}
\providecommand{\Exp}[1]{{\operatorname{exp} \left\{ #1 \right\}}}
\providecommand{\E}[1]{\ensuremath{\mathbb{E} \left[ #1 \right]}}
\providecommand{\CE}[2]{\ensuremath{\mathbb{E} \left[ #1 \middle| #2 \right]}}

\renewcommand{\H}[1]{\ensuremath{H \left( #1 \right)}}
\providecommand{\CH}[2]{\ensuremath{H \left( #1 \middle| #2 \right)}}
\providecommand{\h}[1]{\ensuremath{h \left( #1 \right)}}
\providecommand{\ch}[2]{\ensuremath{h \left( #1 \middle| #2 \right)}}
\providecommand{\MI}[2]{\ensuremath{I \left( #1 ; #2 \right)}}
\providecommand{\CMI}[3]{\ensuremath{I \left( #1 ; #2 \middle| #3 \right)}}


\newcommand{\bm}[1]{\mbox{\boldmath{$#1$}}}
\newcommand{\V}[1]{{\bm{#1}}}
\newcommand{\tv}[1]{\tilde{\V{#1}}}
\renewcommand{\th}{{\tilde h}}
\newcommand{\tvzl}{\tv{w}_{l-1}}
\newcommand{\SNR}{\mathrm{SNR}}
\newcommand{\ENR}{\mathrm{ENR}}
\newcommand{\tSNR}{\widetilde\SNR}
\newcommand{\oSNR}{\overline\SNR}
\newcommand{\ov}{\bar{v}}
\newcommand{\SIR}{\mathrm{SIR}}
\newcommand{\SDR}{\mathrm{SDR}}
\newcommand{\tSDR}{\widetilde\SDR}
\newcommand{\eff}{{\mathrm{eff}}}
\newcommand{\SNReff}{\SNR_\eff}
\newcommand{\SNReq}{\SNR_\mathrm{eq}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\tot}{{\mathrm{tot}}}

\newcommand{\mX}{\mathcal{X}}
\newcommand{\mG}{\mathcal{G}}
\newcommand{\mF}{\mathcal{F}}
% \newcommand{\mH}{\mathcal{H}}
\newcommand{\mH}{H}
\newcommand{\mI}{\mathcal{I}}
\newcommand{\mJ}{\mathcal{J}}
\newcommand{\mS}{\mathcal{S}}
\newcommand{\mY}{\mathcal{Y}}
\newcommand{\mT}{\mathcal{T}}
\newcommand{\mE}{\mathcal{E}}
\newcommand{\mA}{\mathcal{A}}
\newcommand{\mD}{\mathcal{D}}
\newcommand{\mB}{\mathcal{B}}
\newcommand{\mV}{\mathcal{V}}
\newcommand{\mK}{\mathcal{K}}
\newcommand{\mL}{\mathcal{L}}

\providecommand{\hmX}{\hat{\mX}}

\newcommand{\Comment}[1]{}
\newcommand{\old}[1]{}
\newcommand{\rem}[1]{}

\newcommand{\eps}{{\epsilon}}
\newcommand{\teps}{{\tilde{\eps}}}
\newcommand{\veps}{\varepsilon}
\newcommand{\vphi}{\varphi}

\newcommand{\Unif}{\mathrm{Unif}}
\newcommand{\Det}{\mathrm{Deter}}
\newcommand{\Vlike}{\mathrm{V-like}}

\newcommand{\modD}{\: \mathrm{mod} \: \Delta}
\newcommand{\modL}{\: \mathrm{mod} \: \Lambda}
%\newcommand{\modA}{\: \mathrm{mod} \: \mA_\Delta}
\newcommand{\modA}{\modL}
\newcommand{\Neff}{{N_\textrm{eff}^\beta}}
\newcommand{\NeffG}{N_\textrm{eff,G}^\beta}
\newcommand{\opt}{\mathrm{opt}}
\newcommand{\err}{\mathrm{err}}
\newcommand{\MMSE}{{\mathrm{MMSE}}}
\newcommand{\lattice}{\mathrm{lattice}}
\newcommand{\esupport}{\{ -\delta, \delta \}}
\newcommand{\bsupport}{\{ 1 - \delta, 1 + \delta \}}
\newcommand{\Ea}[1]{E_\alpha \left[ {#1} \right]}
\newcommand{\supp}[1]{ \mathrm{Supp} \left\{ #1 \right\} }


\newcommand{\inner}[2]{\left\langle #1, #2 \right\rangle}

\providecommand{\ha}{{\hat{a}}}
\providecommand{\hb}{{\hat{b}}}
\providecommand{\hc}{{\hat{c}}}
\providecommand{\hd}{{\hat{d}}}
\providecommand{\he}{{\hat{e}}}
\providecommand{\hf}{{\hat{f}}}
\providecommand{\hg}{{\hat{g}}}
\providecommand{\hh}{{\hat{h}}}
\providecommand{\hi}{{\hat{i}}}
\providecommand{\hj}{{\hat{j}}}
\providecommand{\hk}{{\hat{k}}}
\providecommand{\hl}{{\hat{l}}}
\providecommand{\hm}{{\hat{m}}}
\providecommand{\hn}{{\hat{n}}}
\providecommand{\ho}{{\hat{o}}}
\providecommand{\hp}{{\hat{p}}}
\providecommand{\hq}{{\hat{q}}}
\providecommand{\hr}{{\hat{r}}}
\providecommand{\hs}{{\hat{s}}}
\providecommand{\ht}{{\hat{t}}}
\providecommand{\hu}{{\hat{u}}}
\providecommand{\hv}{{\hat{v}}}
\providecommand{\hw}{{\hat{w}}}
\providecommand{\hx}{{\hat{x}}}
\providecommand{\hy}{{\hat{y}}}
\providecommand{\hz}{{\hat{z}}}

\providecommand{\hA}{{\hat{A}}}
\providecommand{\hB}{{\hat{B}}}
\providecommand{\hC}{{\hat{C}}}
\providecommand{\hD}{{\hat{D}}}
\providecommand{\hE}{{\hat{E}}}
\providecommand{\hF}{{\hat{F}}}
\providecommand{\hG}{{\hat{G}}}
\providecommand{\hH}{{\hat{H}}}
\providecommand{\hI}{{\hat{I}}}
\providecommand{\hJ}{{\hat{J}}}
\providecommand{\hK}{{\hat{K}}}
\providecommand{\hL}{{\hat{L}}}
\providecommand{\hM}{{\hat{M}}}
\providecommand{\hN}{{\hat{N}}}
\providecommand{\hO}{{\hat{O}}}
\providecommand{\hP}{{\hat{P}}}
\providecommand{\hQ}{{\hat{Q}}}
\providecommand{\hR}{{\hat{R}}}
\providecommand{\hS}{{\hat{S}}}
\providecommand{\hT}{{\hat{T}}}
\providecommand{\hU}{{\hat{U}}}
\providecommand{\hV}{{\hat{V}}}
\providecommand{\hW}{{\hat{W}}}
\providecommand{\hX}{{\hat{X}}}
\providecommand{\hY}{{\hat{Y}}}
\providecommand{\hZ}{{\hat{Z}}}

\newcommand{\tb}{\tilde{b}}
\newcommand{\tW}{\tilde{W}}
\newcommand{\tZ}{\tilde{Z}}
\newcommand{\tq}{\tilde q}
\newcommand{\tg}{\tilde g}
\newcommand{\tm}{{\tilde{m}}}
\newcommand{\tL}{{\tilde L}}
\newcommand{\tw}{\tilde w}
\newcommand{\tX}{\tilde X}
\newcommand{\tgamma}{\tilde \gamma}

\newcommand{\UB}{\mathrm{UB}}
\newcommand{\Ei}{\mathrm{Ei}}

\newcommand{\tA}{\tilde A}
\newcommand{\tC}{\tilde C}
\newcommand{\tDelta}{\tilde \delta}
\newcommand{\tP}{\tilde{P}}
\newcommand{\tE}{\tilde{E}}
\newcommand{\tN}{\tilde{N}}
\newcommand{\tkappa}{\tilde{\kappa}}
\newcommand{\tn}{\tilde{n}}
\newcommand{\htP}{\hat{\tP}}
\newcommand{\htS}{\hat{\tS}}
\providecommand{\tT}{\tilde T}
\newcommand{\tD}{\tilde D}
\newcommand{\td}{\tilde d}
\newcommand{\tH}{\tilde H}
\newcommand{\tU}{\tilde U}
\newcommand{\ts}{\tilde s}
\newcommand{\bts}{\tilde \bs}
\newcommand{\btS}{\tilde \bS}
\newcommand{\tS}{\tilde S}
\newcommand{\oS}{\overline S}
\newcommand{\ty}{\tilde y}
\newcommand{\tty}{\overline{y}}
\providecommand{\tx}{\tilde x}
\providecommand{\tz}{\tilde z}
\newcommand{\tY}{\tilde Y}
\providecommand{\tU}{{\tilde U}}
\newcommand{\trho}{r} %{\lambda} %{{\underline{\rho}}}
\newcommand{\tR}{\tilde R}
\newcommand{\ta}{\tilde a}
\newcommand{\tV}{\tilde V}
\newcommand{\tr}{\tilde r}

\newcommand{\bd}{{\bm d}}
\newcommand{\bD}{{\bf D}}
\newcommand{\bt}{{\bm t}}
\newcommand{\bs}{{\bm s}}
\newcommand{\tinyS}{{\footnotesize \bs}}
\newcommand{\tinyW}{{\footnotesize \bw}}
\newcommand{\by}{{\bm y}}
%\newcommand{\bY}{\bm Y}
\newcommand{\bS}{\text{\bm S}}
\providecommand{\htx}{\hat{\tx}}
\newcommand{\bhS}{{\bf \hat{S}}}
\newcommand{\hbS}{{\bf \hat{S}}}
\newcommand{\hbX}{{\bf \hat{X}}}

\providecommand{\hbs}{\hat{\bs}}

\newcommand{\bn}{{\bm n}}
\newcommand{\bC}{\text{\bf C}}
\newcommand{\bH}{\text{\bf H}}
\newcommand{\bI}{\text{\bf I}}
\newcommand{\bT}{\text{\bf T}}
\newcommand{\bPhi}{{\bf \Phi}}
\newcommand{\bK}{\text{\bf K}}
\providecommand{\bU}{\text{\bf U}}
\providecommand{\bV}{\text{\bf V}}
\providecommand{\tbV}{\tilde{\bV}}
\providecommand{\tbU}{\tilde{\bU}}
\providecommand{\bD}{\text{\bf D}}
\providecommand{\tbD}{\tilde{\bD}}
\providecommand{\bW}{\text{\bf W}}
\newcommand{\bX}{{\bf X}}
\newcommand{\bR}{\mathbf{R}}
\providecommand{\tbT}{\tilde{\bT}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bE}{{\bf E}}
\newcommand{\bx}{{\bm x}}
\providecommand{\bu}{{\bm u}}
\providecommand{\bv}{{\bm v}}
\newcommand{\bY}{{\bf Y}}
\newcommand{\bZ}{{\bf Z}}
\providecommand{\bV}{{\bf V}}
\newcommand{\bz}{{\bm z}}
\newcommand{\ba}{{\bm a}}
\newcommand{\blambda}{{\bm \lambda}}
\providecommand{\be}{{\bm e}}
\newcommand{\bw}{{\bm w}}
\newcommand{\tbw}{\tilde{\bw}}

\newcommand{\bg}{{\bm g}}
\newcommand{\bh}{{\bm h}}

% % \newcommand{\bchi}{{\bm \chi}}
% % \newcommand{\tbchi}{\tilde {\bm \chi}}
% \newcommand{\bchi}{{\mathfrc{x}}}
% \newcommand{\tbchi}{\tilde \bchi}

\newcommand{\cS}{{\mathcal S}}
\newcommand{\cP}{{\mathcal P}}
\newcommand{\cN}{{\mathcal N}}

\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calE}{{\cal E}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calI}{{\cal I}}
\newcommand{\calJ}{{\cal J}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calL}{{\cal L}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\calO}{{\cal O}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calT}{{\cal T}}
\newcommand{\calU}{{\cal U}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calW}{{\cal W}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calY}{{\cal Y}}
\newcommand{\calZ}{{\cal Z}}

\newcommand{\Id}{\mathcal{I}_{\delta}}
%\newcommand{\Ad}{\mathcal{A}_\Delta}
\newcommand{\Ad}{\Lambda}
\newcommand{\THP}{\text{THP}}
\newcommand{\aR}{\alpha_R}
\newcommand{\aT}{\alpha_T}
\newcommand{\aMMSE}{{\alpha_\MMSE}}
\newcommand{\aRMMSE}{{\alpha_R^\MMSE}}
\newcommand{\aTMMSE}{{\alpha_T^\MMSE}}
\newcommand{\naive}{{\text{Na\"ive}}}
\newcommand{\talpha}{{\tilde \alpha}}

\providecommand{\infinity}{\infty}

\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\Norm}[1]{\left\| #1 \right\|}
\newcommand{\Nu}{\mathcal{V}}
\providecommand{\ctg}{ {\rm ctg} }
\providecommand{\ctan}{ {\rm ctg} }
\providecommand{\tg}{ {\rm tg} }
\renewcommand{\tan}{ {\rm tg} }
\providecommand{\sec}{ {\rm sec} }
\providecommand{\cosec}{ {\rm cosec} }
\providecommand{\e}{{\rm e}}
\providecommand{\comment}[1]{}
\newcommand{\thetaapp}{\theta - (\alpha - \varepsilon)}
\providecommand{\norm}[1]{\Norm{#1}}
\providecommand{\Relu}[1]{\mathrm{Relu}\left(#1\right)}


\newcommand{\BC}{{\text{BC}}}
\newcommand{\MAC}{{\text{MAC}}}
\newcommand{\LPF}{{\text{LPF}}}
\newcommand{\RF}{{\text{RF}}}
\newcommand{\AF}{{\text{AF}}}
\newcommand{\DF}{{\text{DF}}}
\newcommand{\CF}{{\text{CF}}}
\providecommand{\BW}{\text{BW}}
\newcommand{\out}{{\text{out}}}
\newcommand{\inn}{{\text{in}}}
\renewcommand{\outer}{{\text{outer}}}
\newcommand{\wh}{{\text{white}}}

\newcommand{\ej}{\e^{j 2 \pi f}}

\newcommand{\beqn}[1]{\begin{eqnarray}\label{#1}}
\newcommand{\eeqn}{\end{eqnarray}}
\newcommand{\beq}[1]{\begin{equation}\label{#1}}
\newcommand{\eeq}{\end{equation}}

\newcommand{\inthalf}[1]{\int_{-\frac{1}{2}}^{\frac{1}{2}} #1 df}
\newcommand{\ejj}{{\mathrm{e}^{j2\pi f}}}

\providecommand{\var}[1]{{\rm Var\left( #1 \right)}}
\providecommand{\ind}{{\perp \hspace{-2.3mm} \perp}}

\newcommand{\upharpoon}{{\upharpoonleft\hspace{-0.05cm}\upharpoonright}}

\providecommand{\Ddef}{\triangleq}

\newcommand{\MSE}{\mathrm{MSE}}
\newcommand{\ML}{\mathrm{ML}}
\newcommand{\MAP}{\mathrm{MAP}}

\newcommand{\tby}{\tilde {\bm y}}
\newcommand{\tbx}{\tilde {\bm x}}
\newcommand{\tbn}{\tilde {\bm n}}
\newcommand{\tbz}{\tilde {\bm z}}
\newcommand{\tbZ}{{\tilde{ \bf Z}}}
\providecommand{\tbX}{{\tilde{ \bf X}}}
\newcommand{\btZ}{{\tilde{ \bf Z}}}
% \newcommand{\cC}{{\cal C}}
\newcommand{\cR}{{\mathcal R}}
\newcommand{\cC}{{\mathcal C}}
\providecommand{\rank}{\text{rank}}
\providecommand{\diag}{\text{diag}}
\providecommand{\qqquad}{\quad \qquad}
\providecommand{\qqqquad}{\qquad \qquad}

\providecommand{\ZF}{\text{ZF}}
\providecommand{\trace}{\text{trace}}
\providecommand{\rel}{\text{rel}}
\providecommand{\half}{\frac{1}{2}}
% % \providecommand{\bfy}{{\bf y}}
% % \providecommand{\bfz}{{\bf z}}
% \providecommand{\bfy}{{\bf \mathfrc{y}}}
% \providecommand{\bfz}{{\bf \mathfrc{z}}}
% \providecommand{\bfx}{{\bf \mathfrc{x}}}
\providecommand{\common}{\text{common}}
\providecommand{\Haug}{\mH^\text{aug}}

\providecommand{\Xcoh}{\bx^\text{C}}
\providecommand{\Xdir}{\bx^\text{D}}
\providecommand{\XCOH}{X^\text{C}}
\providecommand{\XDIR}{X^\text{D}}

%%%% From ITW2012 Full-Duplex paper
\providecommand{\ZF}{\text{ZF}}
\providecommand{\trace}{\text{trace}}
\providecommand{\rel}{\text{rel}}
\providecommand{\src}{\text{t}}
\providecommand{\dst}{\text{r}}
\providecommand{\half}{\frac{1}{2}}

\providecommand{\Xcoh}{\bx^\text{C}}
\providecommand{\Xdir}{\bx^\text{D}}
\providecommand{\xdir}{x^\text{D}}
\providecommand{\xcoh}{x^\text{C}}
\providecommand{\XCOH}{X^\text{C}}
\providecommand{\XDIR}{X^\text{D}}
\providecommand{\bXCOH}{{\bf X^\text{C}}}
\providecommand{\bXDIR}{{\bf X^\text{D}}}
\providecommand{\tty}{\overline{\by}}
\providecommand{\tby}{\tilde {\bm y}}
\providecommand{\tbx}{\tilde {\bm x}}
\providecommand{\tbn}{\tilde {\bm n}}
\providecommand{\tbz}{\tilde {\bm z}}
\providecommand{\ttz}{\overline{\bz}}
\providecommand{\bfy}{{\cal Y}}
\providecommand{\bfz}{{\cal Z}}
\providecommand{\ttz}{\overline{\bz}}
\providecommand{\BdirTx}{B^\text{D}_t}
\providecommand{\BcohTx}{B^\text{C}_t}
\providecommand{\BcohRel}{B^\text{C}_\rel}
\providecommand{\equivalent}{{\text{equiv}}}

%% New parentheses sizes (similar to \bigg ane alike)
\makeatletter
\newcommand{\vast}{\bBigg@{4}}
\newcommand{\Vast}{\bBigg@{5}}
\makeatother

%%%% From ISIT2011 two-way relay paper
\providecommand{\CS}{{\text{CS}}}
\providecommand{\PNC}{{\text{PNC}}}

\newcommand{\opI}{I}
\providecommand{\causalKer}[2]{P(#1 \upupharpoons #2)}
\providecommand{\condCausalKer}[3]{P(#1 \upupharpoons #2 | #3)}
\providecommand{\MI}[2]{{\opI \left( #1 ; #2 \right)}}
\providecommand{\DI}[2]{{\opI \left( #1 \to #2 \right)}}
% \providecommand{\CDI}[3]{{\opI \left( #1 \to #2 | #3\right)}}
% \providecommand{\dsx}[1]{{\delta s_{#1}(t)}}
\providecommand{\dsx}[1]{{s'_{#1}(t)}}

\providecommand{\quant}[1]{{Q_{\Lambda} \left( #1 \right)}}


\providecommand{\KL}[2]{{\bbD \left( #1 \middle\| #2 \right)}}
\providecommand{\CMI}[3]{{\opI \left( #1 ; #2 \middle| #3 \right)}}
\providecommand{\CDI}[3]{{\opI \left( #1 \to #2 \upupharpoons #3 \right)}}
\providecommand{\CKL}[3]{{\bbD \left( #1 \middle\| #2 \middle| #3 \right)}}
\renewcommand{\H}[1]{{H \left( #1 \right)}}
\providecommand{\h}[1]{{h \left( #1 \right)}}
\providecommand{\CH}[2]{{H \left( #1 \middle| #2 \right)}}
\providecommand{\Ch}[2]{{h \left( #1 \middle| #2 \right)}}
\providecommand{\C}[1]{\text{C} \left( #1  \right)}
\newcommand{\hbg}{\hat{\bg}}
\newcommand{\hbgo}{\hat{\bg}^\perp}
\newcommand{\zg}{z_g}
\newcommand{\ug}{u_g}
\newcommand{\vg}{v_g}
\newcommand{\wg}{w_g}
\newcommand{\twg}{\tilde{w}_g}
\newcommand{\zgo}{z_{g^\perp}}

% Cluster
\providecommand{\inter}{{\text{inter}}}
\providecommand{\bHinter}{\bH_{\text{inter}}}
\providecommand{\bxinter}{\bx_{\text{inter}}}

\providecommand{\Cmac}[1]{ \cC_\MAC \left( #1 \right) } 

\providecommand{\dB}{\mathrm{dB}}
\providecommand{\self}{\textrm{self}}
\providecommand{\intra}{\textrm{intra}}
\providecommand{\inter}{\textrm{inter}}

\providecommand{\TWOD}{\text{2D}}
\providecommand{\oD}{\bar{D}}

\providecommand{\bbD}{\mathbb{D}}
\providecommand{\bbE}{\mathbb{E}}
\providecommand{\bbh}{\mathbb{h}}
\providecommand{\bbH}{\mathbb{H}}
\providecommand{\bbI}{\mathbb{I}}
\providecommand{\bbP}{\mathbb{P}}

\providecommand{\E}[1]{\bbE \left[ #1 \right]}
\providecommand{\CE}[2]{\bbE \left[ #1 \middle| #2 \right]}
\providecommand{\Esub}[2]{\bbE_{#1} \left[ #2 \right]}
\providecommand{\CEsub}[3]{\bbE_{#1} \left[ #2 \middle| #3 \right]}
\providecommand{\Pinf}{P_\infty}
\providecommand{\CP}[2]{P \left( #1 \middle| #2 \right)}

\providecommand{\packet}{F}
\providecommand{\PACKET}{a}
% \providecommand{\IF}{\mathrm{if }}
\providecommand{\IF}{}
\providecommand{\AND}{\textrm{ and }}

% \providecommand{\RDF}[2]{\cR \left( \frac{#1}{#2} \right)}
\providecommand{\RDF}[2]{\half \log \left( \frac{#1}{#2} \right)}
\providecommand{\erasure}{\davidsstar}
\providecommand{\Dweight}{D^\mathrm{Weighted}}
\providecommand{\betaut}{b}
\providecommand{\tind}{t}
\providecommand{\twopi}{\tau}

\providecommand{\indind}{k}
\providecommand{\alphat}{\alpha_\tind}
\providecommand{\alphai}{\alpha_\indind}
\providecommand{\alphapr}{\alpha_{\tind-1}}
\providecommand{\Wt}{W_\tind}
\providecommand{\Wpr}{W_{\indind-1}}
\providecommand{\Wi}{W_\indind}
\providecommand{\Rt}{R_\tind}
\providecommand{\rt}{r_\tind}
\providecommand{\Ri}{R_\indind}
\providecommand{\Rpr}{R_{\indind-1}}
\providecommand{\Rone}{R_1}
\providecommand{\Bt}{B_\tind}
\providecommand{\Npackets}{K}

\providecommand{\Eig}{\lambda}
\providecommand{\SNRf}{\SNR_\mathrm{F}}
\providecommand{\SNRb}{\SNR_\mathrm{B}}
\providecommand{\costX}{q}
\providecommand{\costU}{r}

% \renewcommand{\gamma}{\ENR}
\newcommand{\Dzz}{D_\mathrm{ZZ}}
\newcommand{\Dww}{D_\mathrm{WW}}
\providecommand{\Edsgn}{\tE}
\newcommand{\PR}[1]{\Pr\left( #1 \right)}
\newcommand{\CPR}[2]{\Pr\left( #1 \middle| #2 \right)}
\providecommand{\tsigma}{\tilde{\sigma}}
\providecommand{\Nmin}{N_{\min}}

\providecommand{\bullets}{\bullet \bullet \bullet}

\newcommand {\Rh} {R_{\mbox{\tiny h}}}
\newcommand {\Lh} {L_{\mbox{\tiny h}}}
\newcommand {\Mh} {{M_{\mbox{\tiny h}}}}

\newcommand{\dfn}{\triangleq}
\newcommand{\exe}{\doteq}
\providecommand{\dotgeq}{\dot{\geq}}
\newcommand{\gexe}{\dotgeq}

\providecommand{\Exp}[1]{\ensuremath{{\operatorname{exp} \left\{ #1
\right\}}}}

\providecommand{\dotleq}{\mathrel{\dot{\leq}}}
% \providecommand{\dotleq}{\dot{\leq}}
\providecommand{\xto}[2]{\xrightarrow[#2]{#1}}
\providecommand{\Q}[1]{\ensuremath{Q \left( #1 \right)}}

\providecommand{\lrp}[1]{\left( #1 \right)}
\providecommand{\lrr}[1]{\left( #1 \right)}
\providecommand{\lrs}[1]{\left[ #1 \right]}
\providecommand{\lrc}[1]{\left\{ #1 \right\}}

\providecommand{\IV}{V}
\providecommand{\RV}{V}
